Prioritizing Investments in Cybersecurity: Empirical Evidence from an Event Study on the Determinants of Cyberattack Costs

Along with the increasing frequency and severity of cyber incidents, understanding their economic implications is paramount. In this context, listed firms' reactions to cyber incidents are compelling to study since they (i) are a good proxy to estimate the costs borne by other organizations, (ii) have a critical position in the economy, and (iii) have their financial information publicly available. We extract listed firms' cyber incident dates and characteristics from newswire headlines. We use an event study over 2012--2022, using a three-day window around events and standard benchmarks. We find that the magnitude of abnormal returns around cyber incidents is on par with previous studies using newswire or alternative data to identify cyber incidents. Conversely, as we adjust the standard errors accounting for event-induced variance and residual cross-correlation, we find that the previously claimed significance of abnormal returns vanishes. Given these results, we run a horse race of specifications, in which we test for the marginal effects of type of cyber incidents, target firm sector, periods, and their interactions. Data breaches are the most detrimental incident type with an average loss of -1.3\% or (USD -1.9 billion) over the last decade. The health sector is the most sensitive to cyber incidents, with an average loss of -5.21\% (or USD -1.2 billion), and even more so when these are data breaches. Instead, we cannot show any time-varying effect of cyber incidents or a specific effect of the type of news as had previously been advocated.

==> extra/backup.tex <==
%%%%
%Evgueni's part
%%%%



%%%%%%
%Evgueni's part
%%%%%%
\subsubsection{News treatment}

Our study collected news headlines from the Refinitiv Eikon platform, recognized for its comprehensive financial news coverage and its use in previous event analyses, such as \cite{ElGhoul2023} and \cite{su14020852}. This platform can categorize news with a Cybercrime tag, focusing on cyber incidents. Initially, we gathered 106,248 headlines.

To refine this dataset, we selected headlines in English related to listed companies, reducing our pool to 27,244. We further narrowed it down to 12,561 by focusing on North American companies identifiable by their CUSIP. To identify characteristic keywords in cyber incident headlines, we compared 12,297 of these headlines against a normal news corpus using a volcano plot, as illustrated in Figure 6.

A volcano plot contrasts word frequencies between two distinct datasets. The x-axis shows the log2 fold change, indicating the relative frequency shift of words between cybercrime and regular headlines. Words more common in cybercrime headlines have a higher positive value. The y-axis presents the negative log (base 10) of the p-value from a chi-squared test, highlighting the statistical significance of the frequency differences. Words at the top of the plot show significant and substantial frequency changes, thus distinguishing cybercrime headlines from regular news.

Based on this analysis, we identified keywords typically associated with cyber incidents, such as \textit{"breach", "hacker", "cybersecurity", "ransomware", "malware", "leak", "vulnerability", "data", and "attack"}. These terms, though not exhaustive, cover a broad range of cyber incident scenarios (e.g., \textit{[Company Name] is experiencing a [Keyword]}).

Applying these keywords, we refined the headlines to include specific cyber terms and company names, making exceptions for Meta and Alphabet to capture incidents related to Google or Facebook. This process yielded 3,606 headlines.

We then used the MoritzLaurer/DeBERTa-v3-large-mnli-fever-anli-ling-wanli\footnote{Reference at: \href{https://huggingface.co/MoritzLaurer/DeBERTa-v3-large-mnli-fever-anli-ling-wanli}{https://huggingface.co/MoritzLaurer/DeBERTa-v3-large-mnli-fever-anli-ling-wanli}} model from the Hugging Face platform for text entailment, aiming to validate headlines like \textit{[Company Name] has been under a cyber security incident or a cyber attack.} We sought an entailment score above 93\% to underfit the results for later manual evaluation. This model, based on BERT and DeBERTa, is finely tuned on various NLI datasets, offering 885,242 hypothesis-premise pairs, and is highly rated on Hugging Face as of June 6, 2022. This step resulted in 1,465 headlines.

To avoid duplication, we retained only the first headline per day for each company, and headlines at least two months apart for the same company, with exceptions for corporations like Meta, Alphabet, Google, and Apple due to their higher frequency of incidents. This resulted in 368 headlines from my Python script.

Finally, we manually verified these headlines for date accuracy, relevance, and attack type, resulting in a final count of 270 headlines. An example entry is as follows: \newline 

\textit{Company Common Name, Date, Source, RIC, Headline, Exchange Name, TRBC Economic Sector Name, CUSIP, Attack,Data Breach, Software Breach, Cyber breach, Social breach, Ransomware, Shutdown, Twitter breach, Facebook breach, Stolen Funds, Mitigation\newline}

\textit{Adobe Inc, 2012-11-13 19:00:00, RTRS, ADBE.O, "UPDATE 1-Adobe says user forum was breached, takes site offline", unknown, Technology, 00724F101, Data-breach, 1.0,,1.0,,,,,,,\newline}


 All the previously described filtering steps are summarized in figure \ref{fig:sankey_preprocessing}.
 \begin{center}
    [Insert Figure \ref{fig:sankey_preprocessing} here.]
\end{center}




==> extra/cover.tex <==
\begin{titlepage}
    \centering
    \begin{tabularx}{\linewidth}{@{}lXr@{}}
    \hspace{-0.5cm}
    \makecell{\includegraphics[height=2.5cm]{figures/EPFL_Logo_Digital_RGB_PROD.png}}
        &&\makecell{\includegraphics[height=2.5cm]{figures/logo_armasuisse_hoch_komm_SandT_CYD_bold.pdf}}
    \end{tabularx}\\[1.5cm]
    
    \textsc{\LARGE Master's Thesis }\\[0.5cm] % Thesis type
    
    \hrulefill\\[0.2cm] % Horizontal line
    \huge {\bfseries Cybersecurity risks}\\
    \hrulefill \\[1.2cm] % Horizontal line
    
    \begin{minipage}{0.4\textwidth}
    	\begin{flushleft}
    		\large
    		\textit{Author}\\
    		Daniel \textsc{Celeny} % Your name
    	\end{flushleft}
    \end{minipage}
    ~
    \begin{minipage}{0.4\textwidth}
    	\begin{flushright}
    		\large
    		\textit{Academic Supervisor}\\
    		Prof. Pierre \textsc{Collin-Dufresne}
    	\end{flushright}
    \end{minipage}\\[0.5cm]
    
    
    \begin{minipage}{0.4\textwidth}
    	\begin{flushleft}
    	\end{flushleft}
    \end{minipage}
    ~
    \begin{minipage}{0.4\textwidth}
        \begin{flushright}
            \large
    		\textit{Company Supervisors}\\
    		Dr. Alain \textsc{Mermoud}\\
    		Dr. Loïc \textsc{Maréchal}
        \end{flushright}
    \end{minipage}\\[3cm]
    
    
    \Large \textit{A thesis submitted in fulfillment of the requirements\\ for the Master degree in}\\[0.3cm] 
    Financial Engineering\\[1.5cm]
    
    {\Large August 25, 2023}\\[1ex] % Date
\end{titlepage}

==> extra/lit_review_high_freq_event_study.tex <==
\subsubsection{Intraday event studies}

\cite{KappouBrooksWard2010}
%This study focuses on S&P500 inclusions and deletions, examining the impact of potential overnight price adjustment after the announcement of an S&P500 index change. We find evidence of a significant overnight price change that diminishes the returns available to speculators although there are still profits available from the first day after announcement until a few days after the actual event. More importantly, observing the tick-by-tick stock price performance and volume effects on the key days during the event window for the first time, we find evidence of consistent trading patterns during trading hours. A separate analysis of NASDAQ and NYSE listed stocks allows for a detailed examination of the price and volume effect at an intra-day level. We find that index funds appear to cluster their rebalancing activities near to and after the close on the event date, suggesting that they are more concerned with tracking error than profit.


%A note on intraday
\cite{MarshallNguyenVisaltanachoti2019}
%We investigate the specification and power of intraday event study test statistics. Mean, market, and matched firm models generate well-specified return results for a range of intervals up to 60 min around the event. These models detect return shocks equivalent to one spread in one-minute interval data and three spreads in longer intervals. Researchers using intraday return event studies can, therefore, be confident in their robustness. Some volume event study approaches have reasonable power but they are not generally well specified, while a matched-firm approach gives the best combination of specification and power for spread event studies.

also: \cite{BessembinderCarionTuttleVenkataram2016}
%We extend the theory of strategic trading around a predictable liquidation by considering the role of market resiliency. Our model predicts that even a monopolist strategic trader improves market quality and increases liquidator proceeds if trades’ temporary price impacts are quickly reversed, and that competition among strategic traders strictly improves market quality. We provide related empirical evidence by studying prices, liquidity, and individual account trading activity around the large and predictable “roll” trades undertaken by a large exchange-traded fund (ETF). The evidence indicates narrower bid-ask spreads, greater order book depth, and improved resiliency on roll dates. We find that a larger number of individual trading accounts provide liquidity on roll dates, and do not find evidence of the systematic use of predatory strategies. On balance, the theory and evidence imply that traders supply liquidity to rather than exploit predictable trades in resilient markets.


\cite{GregoireMartineau2022}
%We examine the speed and mechanism of the price discovery process following earnings announcements in the after-hours market, a very illiquid trading environment. Prices reflect earnings surprises mostly through changes in quotes rather than through trades. Following positive announcement surprises, ask prices adjust quickly while bid prices are slower to adjust, and vice versa for negative surprises. Returns computed from trade prices underestimate the speed and magnitude of price reactions following announcements relative to returns computed from quotes. These findings emphasize the importance of using quotes and not trade prices when examining intraday price discovery. Because firm announcements such as earnings generally occur in the after-hours market, using quotes is crucial as trading is sparse. We further illustrate the importance of quotes when examining the price discovery process around analyst recommendation revisions.


\cite{Saggu2022}
%Tether Limited has the sole authority to create (mint) and destroy (burn) Tether stablecoins (USD₮). This paper investigates Bitcoin's response to USD₮ supply change events between 2014 and 2021 and identifies an interesting asymmetry between Bitcoin's responses to USD₮ minting and burning events. Bitcoin responds positively to USD₮ minting events over 5- to 30-minute event windows, but this response begins declining after 60 minutes. State-dependence is also demonstrated, with Bitcoin prices exhibiting a greater increase when the corresponding USD₮ minting event coincides with positive investor sentiment and is announced to the public by data service provider, Whale Alert, on Twitter.


\cite{RogersSkinnerZechman2017}
%We describe the process through which the Securities and Exchange Commission (SEC) makes filings “publicly available.” For a sample of Form 4 (insider trade) filings, we show that, during the period we examine, the majority of filings are available to paying subscribers of the SEC's public dissemination system (PDS) feed before they are posted to the EDGAR website, and so provide subscribers and their clients with a private advantage. We show that this advantage translates into an economically significant trading advantage, and prices, volumes, and spreads respond to the news contained in filings beginning around 30 seconds before public posting. These findings indicate that the SEC dissemination process does not always provide a level playing field and that the meaning of publicly available information in capital markets is no longer simple or obvious. In response to our study, the SEC launched an investigation and agreed to eliminate the PDS timing advantage.


\cite{BudishCramtonShim2015}
%The high-frequency trading arms race is a symptom of flawed market design. Instead of the continuous limit order book market design that is currently predominant, we argue that financial exchanges should use frequent batch auctions: uniform price double auctions conducted, for example, every tenth of a second. That is, time should be treated as discrete instead of continuous, and orders should be processed in a batch auction instead of serially. Our argument has three parts. First, we use millisecond-level direct-feed data from exchanges to document a series of stylized facts about how the continuous market works at high-frequency time horizons: (i) correlations completely break down; which (ii) leads to obvious mechanical arbitrage opportunities; and (iii) competition has not affected the size or frequency of the arbitrage opportunities, it has only raised the bar for how fast one has to be to capture them. Second, we introduce a simple theory model which is motivated by and helps explain the empirical facts. The key insight is that obvious mechanical arbitrage opportunities, like those observed in the data, are built into the market design—continuous-time serial-processing implies that even symmetrically observed public information creates arbitrage rents. These rents harm liquidity provision and induce a never-ending socially wasteful arms race for speed. Last, we show that frequent batch auctions directly address the flaws of the continuous limit order book. Discrete time reduces the value of tiny speed advantages, and the auction transforms competition on speed into competition on price. Consequently, frequent batch auctions eliminate the mechanical arbitrage rents, enhance liquidity for investors, and stop the high-frequency trading arms race.


\cite{JiangLikitapiwatMcInish2012}
% We study after-hours trading (AHT), price contributions, and price discovery following quarterly earnings announcements released outside of the normal trading hours. For  Standard & Poor's (S&P) 500 index stocks from 2004-2008, AHT is heightened on an nouncement days. A significant portion of the price change and price discovery occurs  immediately after the earnings releases. Prices in AHT show a large degree of informational efficiency, further demonstrating the importance of price discovery in AHT. We also provide evidence suggesting that firms prefer after-hours earnings announcements, as trades are mainly from informed traders, and those trades are relied upon to convey information to the general public

\cite{ChordiaRollSubrahmanyam2005}
%Daily returns for stocks listed on the New York Exchange (NYSE) are not serially correlated while order imbalances on the same stocks are highly persistent. These empirical facts can be reconciled if sophisticated investors react to order imbalances within the trading day by undertaking enough countervailing trades to remove serial dependence over a daily horizon. How long does this actually take? The pattern of intra-day serial dependence reveals that it takes more than five minutes but less than sixty minutes.


\cite{BusseGreen2002}
%The Morning Call and Midday Call segments on CNBC TV provide a unique opportunity to study the efficient market hypothesis. The segments report analysts’ views about individual stocks and are broadcast when the market is open. We find that prices respond to reports within seconds of initial mention, with positive reports fully incorporated within one minute. Trading intensity doubles in the first minute, with a significant increase in buyer- (seller-) initiated trades after positive (negative) reports. Traders who execute within 15 seconds of the initial mention make small but significant profits by trading on positive reports during the Midday Call.

\cite{KimLinSlovin1997}
%We examine stock price behavior in response to initial coverage, buy recommendations that  are pre-released to important clients before the stock market opens, and find a strong positive  valuation effect at the open. On average, it takes five minutes of trading for NYSE/AMEX  stocks and 15 minutes for NASDAQ stocks to reflect the private information contained in  these analyst recommendations, so when informational asymmetry is high, the centralized  call market is more efficient than a competitive, but fragmented dealer market. Public news  release leaves share prices unaltered. Overall, competition among informed traders causes  private information to be rapidly incorporated into stock prices

\cite{KyleObizhaeva2016}
%Using the intuition that financial markets transfer risks in business time, “market microstructure invariance” is defined as the hypotheses that the distributions of risk transfers (“bets”) and transaction costs are constant across assets when measured per unit of business time. The invariance hypotheses imply that bet size and transaction costs have specific, empirically testable relationships to observable dollar volume and volatility. Portfolio transitions can be viewed as natural experiments for measuring transaction costs, and individual orders can be treated as proxies for bets. Empirical tests based on a data set of 400,000+ portfolio transition orders support the invariance hypotheses. The constants calibrated from structural estimation imply specific predictions for the arrival rate of bets (“market velocity”), the distribution of bet sizes, and transaction costs.


%Also see the literature review of
\cite{Bhattacharya2023W}

==> extra/literature_review_backup.tex <==
\subsection{Event study methodology and critical results}

\subsubsection{Methodology}

Event study methods are heavily employed in all branches of economics. The first modern form of the empirical test to assess the impact of one or several economic events on one or several data series dates back to \cite{BallBrown1968} whose research focuses on the impact assessment of accounting measures changes on stock prices.\footnote{\cite{Dolley1933} is alternately cited as the first author to employ event studies on stock splits.}
\cite{FamaFisherJensenRoll1969} additionally helps to define the modern empirical approach to event studies, as they study the abnormal returns around stock split announcements to falsify the efficient market hypothesis. Although they find significant positive abnormal returns around these announcements, with a market model, they also rationalize them.

While studying the effects of the accuracy of 336 forecast annual earnings disclosures on stock prices over the 1963--1967 period, \cite{Patell1976} additionally introduces a first adjustment in the event study methods. He proceeds by scaling the standard errors used for the t-test of significance by the standard deviation of the estimation period residuals. \cite{BoehmerMusumecciPoulsen1991}  propose a similar adjustment to scale standard errors based on the event-induced variance (see also, \citealp{Savickas2003}). The aforementioned adjustments are the first to account for the event-induced heteroskedasticity of the time series under consideration.

On the other hand, empirical adjustments may be needed to account for the cross-sectional dependence of several firms affected by the same event. To alleviate this effect, \cite{Malatesta1986} proposes the joint generalized least squares approach. Using simulations, he cannot demonstrate, however, that this approach dominates more simplistic cross-sectional dependence treatment. Similarly, \cite{Salinger1992} takes the standpoint that actual abnormal returns must be uncorrelated even though their estimates are not. He derives an adjustment formula for the standard errors using a standard market model approach and a dummy variable. Applying this correction to an event study of post-merger performance, he shows that omitting the adjustment can lead to severe over-rejection of the null hypothesis of no abnormal returns. Similarly, \cite{Karafiath1994} develops the dummy variable approach, which consists of appending a vector of zeros (ones) outside (inside) the event window. This approach enables obtaining abnormal returns in a single step and allows for more straightforward adjustments of the standard errors and an easier interpretation of the residuals.

Another drawback of event studies is that they often rely on daily returns, which are more prone to autocorrelation, leading to underestimation of standard errors. To address this issue, \cite{BrownWarner1985} proposes a series of adjustments and discuss the cross-sectional dependence and event-induced variance issues.

The aforementioned studies and the state-of-the-art methods generally apply to abnormal returns of short windows around the event considered, the cumulative abnormal returns (CAR). However, another strand of literature recognizes issues arising from estimating longer windows around and after the events, the so-called buy-and-hold abnormal returns (BHAR). Advances in the treatment of such BHAR are discussed in \cite{CampbellLoMacKinley1997}
and \cite{KothariWarner2007}.

Finally, \cite{KolariPynnonen2010} develop a t-statistics that summarizes and treats all the aforementioned CAR adjustments proposed. It deals jointly with event-induced variance, cross-correlation, and autocorrelation biases. They test the unbiasedness of their standard errors and the power of the tests in simulations and generate a test that is probably the most effective available parametric test to date.\footnote{This literature review voluntarily skips the minor literature on non-parametric tests. See, \textit{e.g.}, the non-parametric rank test of \cite{KolariPynnonen2011}.}\footnote{Also see, \cite{LeeVarela1997}, for tests of the different available standard errors adjustments.}.

\subsubsection{Critical results}

%Stock split
One of the most scrutinized and oldest documented market anomalies is that of stock-split announcements. \cite{FamaFisherJensenRoll1969} are the first to employ event studies in their modern form to study these effects. They find significant positive abnormal reactions around announcements, which would undermine the efficient market hypothesis. However, they also rationalize this effect, arguing that stock splits are generally associated with favorable expectations about future dividends. Instead, \cite{Copeland1979} justifies this effect because liquidity, and hence returns, increases when prices remain bounded in magnitude.

A second debate concerns the effects of stock additions and deletions from indices. In particular, since investment funds or exchange-traded funds must replicate the performance of these indices for their clients, they must also buy (sell) the newly listed (delisted) asset from the index. Event studies are in perfect adequation to study these effects since they generally concern heavily traded stocks and because these events are frequent. \cite{Shleifer1986} finds that stock addition in the S\&P 500 index experience significant positive abnormal returns. He additionally focuses on the temporary and permanent component of this effect and concludes that this effect is circumvented to temporary \quotes{price pressure} from funds' addition to their portfolio and that it is not an accreditation for quality, which in turn would generate a permanent price increase. \cite{HarrisGurel1986} also find support for the price pressure hypothesis, as they identify average abnormal returns of around 3\% immediately after a stock addition, but which are almost fully reversed two weeks after the addition. \cite{ShleiferVishny1997} explain this time for reversal by introducing the concept of limit to arbitrage. They argue that even this simple arbitrage may be risky and that it entails the use of capital. Thus, price pressure effects may exist temporarily around stock addition before prices revert to their fundamental value. Finally, \cite{KaulMehrotraMorck2000} use the Toronto Stock Exchange 300 Index and the study of a single event, the concurrent revision of 31 stocks' index weights. They find significant abnormal returns of around 2.3\% in magnitude. Unlike the aforementioned studies, they cannot identify any price reversal following this event, which conveyed no information regarding affected stocks.

%Regulation enforcement
\cite{Jaffe1974} uses event studies to assess the effects of regulation enforcement regarding insider trading. He focuses on the Securities and Exchange Act of 1933--1934 and the following legal cases. The selected events are, therefore, legal decisions regarding insiders and the effects on insider trades. He could not find any change in behavior following cases, thus pointing to insufficient law enforcement.

Other use cases for event study methods include the post-earnings announcement drift, studied by \cite{Sadka2006}, among others, but also the price effects of secondary distributions and seasoned equities, empirically studied by \cite{MikkelsonPartch1985}, and \cite{KalayShimrat1987}, respectively. The former authors observe a negative price pressure around secondary distribution announcements. They subsequently explain the variations in price decreases and find that the effects are more significant for distributions from officers and directors and positively relate to the distribution sizes. The latter authors also uncover adverse price pressure effects around seasoned equities and, instead, relate the effect to the fact that seasoned equities carry negative information. \cite{MitchellPulvinoStafford2004} study the effects of around 2,130 mergers over the 1994--2000 period. They find positive price pressure effects, but which are short-lived. In another context, \cite{Jin2006} examines how capital gains tax prevents investors from selling, moving stock prices upward from their fundamentals. He additionally relates this effect to the size of the capital gains. Finally, \cite{HendersonPearsonWang2015} study commodity-linked notes issuance and their effects on their underlying commodity futures market. Again, the events are not associated with any new information. As for stock additions and deletions, these issuances generate considerable pressure on commodity prices.

Few papers study non-financial data or non-financial related events as determinants of an \quotes{event} for stock returns. If they do, this is generally in the context of a single event concurrently affecting several or all firms. In this context, Cyber-events are no exceptions. The following section lists the small but picking-up literature analyzing cyber-events through the lenses of event studies on financial markets.

\subsection{Cyber incident costs}

\subsubsection{Abnormal returns around cyber incidents}

\cite{GordonLoebZhou2011} assess the impact of information security breaches on stock returns by estimating CARs over a three-day event window centered on news of cybersecurity incidents. They find that news about information security breaches generates significant negative CARs for publicly traded firms. They additionally uncover a significant downward shift in the impact of security breaches in the post-9/11 sub-period. They interpret these findings with a shift in investors' attitudes towards cyber breaches. In a similar study, \cite{CampbellGordonLoebZhou2003} uncover highly significant (non-significant) negative CARs for information security breaches (not) involving unauthorized access to confidential data. \cite{JohnsonKangLawson2017} also show that, on average, publicly traded firms in the U.S. face CARs of about -0.37\% over a data breach. Additionally, breaches resulting from payment card fraud contribute more to negative abnormal returns than other breach types. Lastly, they find a positive link between these CARs' magnitude and the card breach' size.

\cite{LendingMinnickSchorno2018} relate corporate governance and social responsibility to the probability of data breaches. Measuring changes in stock returns after breaches, they uncover a persistent effect of –3.5\% of one-year BHAR. They additionally find that banks with breaches have significant decreases in deposits, while non-banks experience large sales decreases. \cite{Tosun2021} studies in both the short- and the long-run how financial markets react to unexpected corporate security breaches. He uncovers that market participants anticipate negative changes in stock prices while analyzing measures of selling pressure and liquidity. However, the negative effect is significantly negative only the day following the security breach public announcements and is linked to an adverse impact on the firm reputation. \cite{KamiyaJun-KooJungminMilidonisStulz2021} find additional support for a reputation loss of targeted firms through a drop in credit ratings or a decrease in sales growth.

%Municipal bonds
\cite{AndreadisKalotychouLoucaLundbladMakridis2023} investigate how information dissemination about cyberattacks through major news sources affects municipalities' access to finance, particularly in the municipal bond market. Using a differences-in-differences framework, they show that an increase in the number of cyberattacks covered by news articles at the county level and the corresponding number of cyberattack news articles has a significant adverse impact on municipal bond yields. A 1\% rise in the number of cyberattacks covered in news articles results in offering yields increasing by 3.7 to 5.9 basis points, depending on the level of cyberattack exposure. \cite{JensenPaine2023} use data on municipal IT investments, ransomware attacks, and bond performance. They cannot find an immediate impact on bond yields within 30 days of a cyberattack. However, over the subsequent 24 months post-cyberattack, municipal bond yields gradually decreased while IT spending increased. They argue that this decline in bond yields is driven by a reduction in cyber risk due to increased IT investment.

%event study style with disclosures
\cite{GordonLoebSohail2010} examines how voluntary information security disclosures impact firm value, using a dataset of 1,641 firms that disclose such information and 19,266 that do not. They find that these disclosures can reduce litigation costs and lower a firm's cost of capital by reducing information asymmetry between management and investors. They find a positive relationship between voluntary information security disclosures and firm value. Firms that disclose this information also exhibit narrower bid-ask spreads than those that do not. \cite{HilarySegalZhang2016W} also study cyber risk disclosures and uncover that the market reaction to cyber breaches is statistically significant but economically narrow.

\subsubsection{Other methods for cyberattacks' costs estimation}

\cite{Bouveret2018W} studies the global cyber risk for the financial sector and the various types of cyber incidents. Using a Value at Risk (VaR) framework, he uncovers an average country loss due to cyberattacks of USD 97 bn and a VaR between USD 147 and 201 bn. He argues that there exist essential potential aggregated losses in the financial sector, several orders of magnitude higher than what the cyber insurance market could cover. \cite{Romanosky2016}) delves into the nature and expenses related to cyber events. His analysis of a dataset comprising over 12,000 incidents reveals a skewed cost distribution, with an average cost of USD 6 mln and a median cost of USD 170,000, akin to a typical annual IT security budget for firms. This leads to the hypothesis that firms may be operating at an optimally secure level due to the relatively low costs, thus investing modestly in data protection measures. Other related studies include, \textit{e.g.}, \cite{AndersonBartonBohmeClaytonEetenLeviMooreSavage2013,AndersonBartonBoehmeClaytonGananGrassoLeviMooreVasek2019}.

%asset pricing perspective
A last strand of research in finance and cybersecurity uses asset pricing techniques and the cross-sectional analysis of listed stocks. Even though this literature relates more to the perceived risk than actual realization, this literature is worth mentioning and includes

\cite{FlorackisLoucaMichaelyWeber2023} develop a text-based cyber risk measurement using a section of 10-K statements called \quotes{Item 1. A Risk Factors} They extract cyber risk-related sentences from this section using a predefined list of keywords and focus the analysis on these sentences. To assess a firm's cybersecurity exposure, they compare its cybersecurity-related sentences with those of recently hacked firms, computing the average similarity. They find that firms with high exposure tend to have higher average returns but perform worse during periods of elevated cyber risk. In a similar study, \cite{JamilovReyTahoun2021W} use quarterly earnings calls data. They create a cyber risk metric by assessing the frequency of cyber-related keywords in these calls. To capture cyber shocks, they compute a factor by calculating the monthly average cyber risk score for firms with non-zero scores and fitting an $AR(1)$ model to the time series, subsequently extracting the residuals. This factor exhibits a structured pattern within the firm-level cybersecurity metric, as evidenced by the average annual return of -3.3\% on a long-short portfolio based on its cybersecurity beta. Additional studies on this picking up literature include: \cite{JiangKhannaYangZhou2023,LiuMarshXiao2022W,CelenyMaréchal2023}.

Hence, we define our null hypotheses as follows:
\begin{itemize}
    \item $H_1$: Cyber incidents do not affect firms' returns adjusted for standard financial benchmarks.

    \item $H_2$: Standard errors are insensitive to the sophistication of the estimation taking into account cross-correlation and event-induced variance.

    \item $H_3$: The impacts of cyber incidents are homogeneous in terms of:
    \begin{itemize}
        \item $H_{3a}$: type of cyber incidents (attackers' origin, firm deficiency, data breach, attack sophistication, attack common to several firms, or number of firms' users/customers compromised)
        \item $H_{3b}$: sector of target firms
        \item $H_{3c}$: characteristics of target firms (size, book-to-market ratios, R\&D intensity, industry.)
        \item $H_{3d}$: time of the cyber incidents in the sample.
    \end{itemize}

    \item $H_4$: The impact of cyber incidents is similar irrespective of the reporting source of the news.
\end{itemize}

==> sections/tables_and_figures.tex <==
\phantom{test}
\vspace{25mm}
\begin{figure}[h]
    \noindent\makebox[\textwidth]{%
    \includegraphics[width=\textwidth]{figures/3_data/cyber_volcano_plot.png}
    }
     \caption{\textbf{Volcano plot of cyber incident headlines against normal headlines}}\bigskip
     \footnotesize{Volcano plot of a normal news corpus against a cybercrime news corpus. The population of both samples is 12,297 and is extracted from Refinitiv. The x-axis represents a log2 fold change, while the y-axis depicts the negative logarithm (base 10) of the p-value derived from a chi-squared test. The x and y thresholds are set to select the relevant keywords optimally.}
     \label{fig:volcano}
\end{figure}


\clearpage
\begin{figure}
    \noindent\makebox[\textwidth]{%
    \includegraphics[width=\textwidth]{figures/3_data/sankey_data_processing_steps.png}
    }
     \caption{\textbf{Filtering process of cyber incident headlines}}\bigskip
     \footnotesize{This diagram depicts the filtering steps of the original cyber incident headline set from Refinitiv. We only keep headlines in English that mention listed companies with an identifier (RIC). Next, we keep North American listed companies that have a CUSIP. We filter based on cyber incident keywords. We subsequently check whether the headline is a premise to the following entailment question: \quotes{[Company Name] has been under a cyber security incident or a cyberattack.} We additionally keep the earliest headline per day and company. These must be two months apart for a given company (starting with the earliest). Finally, we manually change the dates and drop headlines that are not about a cyber incident or are not the first to mention it.}
     \label{fig:sankey_preprocessing}
\end{figure}


\clearpage
\begin{figure}
    \noindent\makebox[\textwidth]{%
    \includegraphics[width=\textwidth]{figures/4_methodology/sankey_events.png}
    }
     \caption{\textbf{Evolution of the number of incidents}}\bigskip
     \footnotesize{In step 1, we drop all firms not in the WRDS database. In step 2, we drop all incidents of cybersecurity-providing firms. In step 3, we drop incidents where the firm's market capitalization is lower than \$300 million, the firm is not listed during the incident, the incident is in 2023, or the incident window is larger than five days. In step 4, we drop all firms not listed between 2013.12.19 and 2022.10.13 and/or whose cyber incident(s) did not occur between those dates.}
     \label{fig:sankey_events}
\end{figure}


\clearpage
\begin{figure}
    \noindent\makebox[\textwidth]{%
    \includegraphics[width=\textwidth]{figures/4_methodology/sankey_firms.png}
    }
     \caption{\textbf{Evolution of the number of firms}}\bigskip
     \footnotesize{In step 1, we drop all firms not in the WRDS database. In step 2, we drop all incidents of cybersecurity-providing firms. In step 3, we drop incidents where the firm's market capitalization is lower than \$300 million, the firm is not listed during the incident, the incident is in 2023, or the incident window is larger than five days. In step 4, we drop all firms not listed between 2013.12.19 and 2022.10.13 and/or whose cyber incident(s) did not occur between those dates.}
     \label{fig:sankey_firms}
\end{figure}


\clearpage
\begin{figure}
    \noindent\makebox[\textwidth]{%
    \includegraphics[width=0.8\textwidth]{figures/4_methodology/industry_dist.png}
    }
     \caption{\textbf{Sector distribution}}\bigskip
     \footnotesize{Sector distribution of the firms remaining after step 3 on Figure \ref{fig:sankey_firms}. We use Refinitiv's sector classification.}
     \label{fig:indsutry_dist}
\end{figure}


\clearpage
\begin{figure}
    \noindent\makebox[\textwidth]{%
    \includegraphics[width=0.8\textwidth]{figures/4_methodology/attack_dist.png}
    }
     \caption{\textbf{Attack distribution}}\bigskip
     \footnotesize{Distribution of the different types of attacks of the incidents remaining after step 3 on Figure \ref{fig:sankey_events}. The \quotes{Other} category regroups the Cyber Breach (1.93\%) and Stolen Funds (1.93\%) categories.}
     \label{fig:attack_dist}
\end{figure}


\clearpage
\begin{figure}
    \noindent\makebox[1.1\textwidth]{%
    \includegraphics[width=0.75\textwidth]{figures/5_results/SURE_correlation.png}
    }
     \caption{\textbf{Correlation of residuals}}\bigskip
     \footnotesize{Correlation matrix of residuals, obtained by estimating Eq. \ref{eq:AR_regression}.}
     \label{fig:residual_corr}
\end{figure}


\clearpage
\begin{table}
    \noindent\makebox[\textwidth]{%
    \begin{tabular}{p{6cm}cccccc}
        %\toprule
        & \multicolumn{3}{c}{Zero-benchmark} & \multicolumn{3}{c}{FF3 benchmark} \\
        \cmidrule(lr){2-4}
        \cmidrule(lr){5-7}
        & OLS & OLS limited & SUR & OLS & OLS limited & SUR  \\
        \midrule 
        $\overline{CAR}$ & -0.89\% & -0.88\% & -0.79\% & -0.74\% &  -0.84\% & -0.78\% \\
        \\
        Unadjusted t-stat & -1.949 & -2.258 & -2.325 & -1.856 & -2.579 & -2.434 \\
        ADJ-PATELL & - & -0.704 & -0.455 & - & -2.095 & -1.807\\
        ADJ-BMP & -0.157 & -0.323 & -0.273 & -0.698 & -1.226 & -1.033\\
        \midrule
        Number of incidents & 167 & 126 & 126 & 167 & 126 & 126 \\
        Number of days in regression & - & 2219 & 2219 & - & 2219 & 2219\\ 
        \bottomrule
    \end{tabular}
    }
    \caption{\textbf{Average CAR and t-stats}}\bigskip
    \footnotesize{$\overline{CAR}$ is the average cumulative abnormal return over a three-day window around the incidents, relative to the three-factor model of Fama and French \cite{FamaFrench1992}. ADJ-BMP and ADJ-PATELL refer to the adjusted statistics of the same name from Kolari and Pynnonen (2010) \cite{KolariPynnonen2010}. The ADJ-PATELL statistic is cross-correlation-adjusted, and the ADJ-BMP statistic is cross-correlation and volatility-adjusted. The OLS model allows for the number of days in the regression to differ for each firm, and the average number of days is 2398. The OLS limited model is the OLS model restricted to the same period, the same subset of firms, and the same incidents as the SUR model. The zero-benchmark model is shown in Eq. \ref{eq:AR_regression_zb} and the FF3 benchmark model is shown in Eq. \ref{eq:AR_regression}.}
    \label{tab:average_car_tstat}
\end{table}


\clearpage
\begin{figure}
    \noindent\makebox[\textwidth]{%
    \includegraphics[width=\textwidth]{figures/5_results/AAR.png}
    }
     \caption{\textbf{Average abnormal returns}}\bigskip
     \footnotesize{Average abnormal daily returns in an 11-day window centered on the cyber incidents. Day 0 is the day of the cyber incident. The OLS limited model is the OLS model restricted to the same period, the same subset of firms and incidents as the SUR model. Abnormal returns are computed with the three-factor model of Fama and French, following Eq. \ref{eq:AR_regression} \cite{FamaFrench1992}.}
     \label{fig:AAR}
\end{figure}

\clearpage
\begin{figure}
    \noindent\makebox[\textwidth]{%
    \includegraphics[width=\textwidth]{figures/5_results/CAAR.png}
    }
     \caption{\textbf{Cumulative average abnormal returns}}\bigskip
     \footnotesize{Cumulative average abnormal daily returns in an 11-day window centered on the cyber incidents. Day 0 is the day of the cyber incident. The OLS limited model is the OLS model restricted to the same period, the same subset of firms and incidents as the SUR model. Abnormal returns are computed with the three-factor model of Fama and French, following Eq. \ref{eq:AR_regression} \cite{FamaFrench1992}.}
     \label{fig:CAAR}
\end{figure}


\clearpage
\begin{table}
    \begin{adjustbox}{width= 0.38\textwidth,center}
    \begin{tabular}{lcc}
        \hline
        \hline
        \multicolumn{3}{c}{Dependent variable: CAR}\\
        \hline
        & OLS & SUR \\
        \cmidrule(lr){2-2}
        \cmidrule(lr){3-3}
        & Model 4 & Model 4\\
        \hline
        Reuters & \textbf{0.186} & \textbf{-0.477}\\
        & [0.219] & [-0.718] \\
        Twitter & \textbf{-0.843} & \textbf{-1.029}\\
        & [-0.313] & [-0.549] \\
        Other & \textbf{-0.840} & \textbf{-0.472}\\
        & [-1.239] & [-0.927]\\        
        \hline
        Observations & 167 & 126\\
        R-squared & 0.001 & 0.006\\
        \hline
        \hline
    \end{tabular}
    \end{adjustbox}
\caption{\textbf{Determinants of CARs - News source}}\bigskip
\footnotesize{Results of regressions of the CARs on the news source. t-statistics are reported in brackets. The CARs are multiplied by 100. The first column uses the CARs obtained using OLS regressions, and the other column uses the CARs obtained with SUR.}
\label{tab:CAR_on_source}
\end{table}


\clearpage
\begin{table}
    \begin{adjustbox}{width= 0.60\textwidth,center}
    \begin{tabular}{lcccc}
        \hline
        \hline
        \multicolumn{5}{c}{Dependent variable: CAR}\\
        \hline
        & \multicolumn{2}{c}{OLS} & \multicolumn{2}{c}{SUR}\\
        \cmidrule(lr){2-3}
        \cmidrule(lr){4-5}
        & Model 1 & Model 2 & Model 1 & Model 2\\
        \hline
        Data breach & \textbf{-1.287}$^{*}$ & \textbf{0.261} & \textbf{-1.178}$^{**}$ & \textbf{-1.220}\\
        & [-1.907] & [0.167] & [-2.106] & [-1.013]\\
        Software breach & \textbf{-0.380} & & \textbf{-0.178}\\
        & [-0.480] & & [-0.290]\\
        Cyber breach & \textbf{1.152} & & \textbf{1.270}\\
        & [0.438] & & [0.349]\\
        Social breach & \textbf{0.081} & & \textbf{-0.086}\\
        & [0.045] & & [-0.061]\\
        Ransomware & \textbf{0.395} & & \textbf{-0.851}\\
        & [0.258] & & [-0.705]\\
        Shutdown & \textbf{-0.436} & & \textbf{-0.753}\\
        & [-0.041] & & [-0.747]\\
        Twitter breach & \textbf{-0.846} & & \textbf{-0.683}\\
        & [-0.070] & & [-0.817]\\
        Facebook breach & \textbf{2.378} & & \textbf{1.786}\\
        & [1.010] & & [1.096]\\
        Stolen Funds & \textbf{0.362} & & \textbf{-0.617}\\
        & [0.135] & & [-0.231]\\
        Mitigation  & \textbf{1.762} & & \textbf{1.764}\\
        & [0.748] & & [1.083]\\
        Other & & \textbf{1.362} & & \textbf{0.422}\\
        & & [0.960] & & [0.360]\\
        \\
        Technology & & \textbf{-2.172} & & \textbf{-0.923}\\
        & & [-1.413] & & [-0.732]\\
        Consumer products & & \textbf{1.561} & & \textbf{-0.272}\\
        & & [0.793] & & [-0.166]\\
        Financials & & \textbf{-3.825} & & \textbf{0.955}\\
        & & [-0.722] & & [0.856]\\
        Healthcare & & \textbf{-5.210} & & \textbf{1.399}\\
        & & [-1.594] & & [0.500]\\
        Industrials & & \textbf{-1.713} & & \textbf{-3.471}\\
        & & [-0.680] & & [-1.455]\\
        \\
        Data breach * Technology & & \textbf{0.434} & & \textbf{0.329}\\
        & & [0.285] & & [0.270]\\
        Data breach * Consumer products & & \textbf{-2.341} & & \textbf{0.599}\\
        & & [-1.173] & & [0.380]\\
        Data breach * Financials & & \textbf{3.799} & & \textbf{0.955}\\
        & & [0.799]  & & [0.856]\\
        Data breach * Healthcare & & \textbf{-0.251} & & \textbf{-7.069}$^{*}$\\
        & & [-0.080] & & [-1.917]\\
        Data breach * Industrials & & \textbf{-1.381} & & \textbf{3.966}$^{*}$\\
        & & [-0.524] & & [1.708]\\
        \hline
        Observations & 167 & 167 & 126 & 126\\
        R-squared & 0.042 & 0.106 & 0.085 & 0.109\\
        \hline
        \hline
    \end{tabular}
    \end{adjustbox}
\caption{\textbf{Determinants of CARs - Incident type and target sector}}\bigskip
\footnotesize{Results of regressions of the CARs on the firm's sector and the type of the incident. t-statistics are reported in brackets. The CARs are multiplied by 100. \quotes{Consumer products} regroups the consumer cyclical and consumer non-cyclical sectors. The first two columns use the CARs obtained using OLS regressions, and the other two columns use the CARs obtained with SUR. *, **, and *** indicate significance at the 10\%, 5\% and 1\% levels, respectively.}
\label{tab:CAR_on_sector_type}
\end{table}


\clearpage
\begin{table}
    \begin{adjustbox}{width= 0.38\textwidth,center}
    \begin{tabular}{lcc}
        \hline
        \hline
        \multicolumn{3}{c}{Dependent variable: CAR}\\
        \hline
        & OLS & SUR \\
        \cmidrule(lr){2-2}
        \cmidrule(lr){3-3}
        & Model 3 & Model 3\\
        \hline
        2013 & \textbf{0.557} & -\\
        & [0.336]& -\\
        2014 & \textbf{-0.029} & -\\
        & [-0.017] & -\\
        2015 & \textbf{-1.109} & \textbf{-0.899}\\
        & [-0.598] & [-0.659]\\
        2016 & \textbf{-1.019} & \textbf{-1.760}$^{*}$\\
        & [-0.727] & [-1.756]\\
        2017 & \textbf{-0.324} & \textbf{-0.662}\\
        & [-0.262] & [-0.709]\\
        2018 & \textbf{-1.536} & \textbf{-1.790}$^{**}$\\
        & [-1.243] & [-1.981]\\
        2019 & \textbf{-0.651} & \textbf{-0.028}\\
        & [-0.430] & [-0.022]\\
        2020 & \textbf{-0.268} & \textbf{0.446}\\
        & [-0.260] & [0.550]\\
        2021 & \textbf{-1.799} & \textbf{-1.527}\\
        & [-1.456] & [-1.581]\\
        2022 & \textbf{-1.716}$^{*}$ & \textbf{-0.228}\\
        & [-1.822] & [-0.309]\\
        \hline
        Observations & 167 & 126\\
        R-squared & 0.050 & 0.084\\
        \hline
        \hline
    \end{tabular}
    \end{adjustbox}
\caption{\textbf{Determinants of CARs - Incident year}}\bigskip
\footnotesize{Results of regressions of the CARs on years. t-statistics are reported in brackets. The CARs are multiplied by 100. The first column uses the CARs obtained using OLS regressions, and the other column uses the CARs obtained with SUR. *, **, and *** indicate significance at the 10\%, 5\% and 1\% levels, respectively.}
\label{tab:CAR_on_years}
\end{table}


\clearpage
\begin{table}
    \begin{adjustbox}{width= 0.38\textwidth,center}
    \begin{tabular}{lcc}
        \hline
        \hline
        \multicolumn{3}{c}{Dependent variable: CAR}\\
        \hline
        & OLS & SUR \\
        \cmidrule(lr){2-2}
        \cmidrule(lr){3-3}
        & Model 5 & Model 5\\
        \hline
        Constant & \textbf{-6.040} & \textbf{-7.872}$^*$\\
        & [-1.177] & [-1.682] \\
        Firm size (ln) & \textbf{0.206} & \textbf{0.348}$^*$\\
        & [0.994] & [1.881] \\
        Firm Age (ln) & \textbf{0.155} & \textbf{-0.414}\\
        & [0.741] & [-0.946] \\
        Book to market & \textbf{-0.065} & \textbf{-0.035}\\
        & [-0.644] & [-0.247] \\
        Price to earnings & \textbf{0.001} & \textbf{-0.015}$^{**}$\\
        & [0.115] & [-2.164] \\
        \hline
        Observations & 150 & 117\\
        R-squared & 0.017 & 0.075\\
        \hline
        \hline
    \end{tabular}
    \end{adjustbox}
\caption{\textbf{Determinants of CARs - Firm characteristics}}\bigskip
\footnotesize{Results of regressions of the CARs on firm characteristics. t-statistics are reported in brackets. The CARs are multiplied by 100. The first column uses the CARs obtained using OLS regressions, and the other column uses the CARs obtained with SUR. Certain observations were dropped due to missing accounting data. *, **, and *** indicate significance at the 10\%, 5\% and 1\% levels, respectively.}
\label{tab:CAR_on_characteristics}
\end{table}
